Computing Nash Equilibrium in Wireless Ad Hoc Networks: A Simulation-Based Approach

This paper studies the problem of computing Nash equilibrium in wireless networks modeled by Weighted Timed Automata. Such formalism comes together with a logic that can be used to describe complex features such as timed energy constraints. Our contribution is a method for solving this problem using Statistical Model Checking. The method has been implemented in UPPAAL model checker and has been applied to the analysis of Aloha CSMA/CD and IEEE 802.15.4 CSMA/CA protocols.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{J. Reich and B. Finkbeiner (Eds.): 2nd Int'l Workshop\\
on Interactions, Games and Protocols 2012 (IWIGP2012)\\
EPTCS 78, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.78.1}{10.4204/EPTCS.78.1}}

